Double categories of relations relative to factorisation systems

We relativise double categories of relations to stable orthogonal factorisation systems. Furthermore, we present the characterisation of the relative double categories of relations in two ways. The first utilises a generalised comprehension scheme, and the second focuses on a specific class of vertical arrows defined solely double-categorically. We organise diverse classes of double categories of relations and correlate them with significant classes of factorisation systems. Our framework embraces double categories of spans and double categories of relations on regular categories, which we meticulously compare to existing work on the characterisations of bicategories and double categories of spans and relations.

==> newsubsections/LocallyPosetal.tex <==
\subsection{Locally Posetality and Properness}\label{sec:locallyposetal}

\begin{definition}
	Let $\dbl{D}$ be a cartesian double category and $\zero{M}$ be a class of
	vertical arrows in $\dbl{D}$.
	For a horizontal arrow $p\colon X\sto Y$,
	we say $p$ has \emph{$\zero{M}$-presentation}
	if there exists an vertical arrow
	$\langle f,g\rangle\colon A\to X\times Y$ in $\zero{M}$ such that
	there exists an opcartesian cell of the following form.
	\[
		\begin{tikzcd}[column sep=small]
				&
				A
				\ar[ld, "f"']
				\ar[rd, "g"]
					&
			\\
			X
			\doublecell[rr, shift left=2.5ex]{\opcart}
			\sar[rr, "p"']
				&
					&
					Y
		\end{tikzcd}
	\]
	We say $\dbl{D}$ has \emph{$\zero{M}$-presentations} if
	every horizontal arrow has $\zero{M}$-presentation.

	We say $\dbl{D}$ has \emph{left-sided $\zero{M}$-presentations} if
	every horizontal arrow to the terminal object has $\zero{M}$-presentation.
	Note that even if $\dbl{D}$ is not cartesian but with vertical terminal
	this terminology makes sense.
\end{definition}

\begin{proposition}
	Any split mono is an inclusion in any locally posetal double category.
	In particular, any diagonal is an inclusion in any locally posetal cartesian double category.
\end{proposition}
\begin{proof}
	Let $i \colon  A \to B$ be a split mono.
	It suffices to show that for each parallel pair of arrows $f, g\colon X \to A$,
	a cell $f\leq g$ exists if and only if so does $f;i\leq g;i$.
	The only-if part is trivial,
	and if part is obtained by post-composing the retraction of $i$.
\end{proof}

\begin{corollary}
	For a locally posetal cartesian double category $\dbl{D}$
	and an object $X\in\dbl{D}$,
	$X$ is discrete if and only if the right-hand square
	in \Cref{dgm:Discrete} satisfies the Beck-Chevalley condition.
\end{corollary}

For a locally posetal 2-category $\bi{B}$, we say $\bi{B}$ is \textit{discrete} if $\Map(\bi{B})$ is also discrete.

\begin{proposition}
	Any locally posetal discrete cartesian equipment is unit-pure.
\end{proposition}
\begin{proof}
	Let $\dbl{D}$ be a locally posetal discrete cartesian equipment,
	and $f, g\colon X\to Y$ be parallel vertical arrows in $\dbl{D}$.
	Suppose there exists a vertical cell $f \leq g$ and it suffices to show that
	there also exists a vertical cell $g \leq f$.
	Since $\times$ is a double functor, we obtain a vertical cell
	$f\times f\times g\leq f\times g\times g$
	and hence $\langle f, f, g\rangle\leq\langle f, g, g\rangle$.
	This cell is described as a vertical cell on the left below.
	Since
	$(\id\times\Delta)_!(\Delta\times\id)^*%
	\cong\Delta^*\Delta_!%
	\cong(\Delta\times\id)_!(\id\times\Delta)^*$, we obtain another cell on
	the right below, which is equivalent to
	$\langle f, g, g\rangle\leq\langle f, f, g\rangle$.
	In particular, we obtain $g\leq f$ by post-composing the second projection.
	\[
		\begin{tikzcd}[column sep = small]
				&
				X
				\ar[ld,"\mmbox{\langle f,g\rangle}"']
				\ar[rd,"\mmbox{\langle f,g\rangle}"]
					&
			\\
			Y\times Y
			\ar[rd,"\Delta\times\id"']
				&
				\leq
					&
					Y\times Y
					\ar[ld,"\id\times\Delta"]
			\\
				&
				Y\times Y\times Y
					&
		\end{tikzcd}
		\hspace{5ex}
		\begin{tikzcd}[column sep = small]
				&
				X
				\ar[ld,"\mmbox{\langle f,g\rangle}"']
				\ar[rd,"\mmbox{\langle f,g\rangle}"]
					&
			\\
			Y\times Y
			\ar[rd,"\id\times\Delta"']
				&
				\leq
					&
					Y\times Y
					\ar[ld,"\Delta\times\id"]
			\\
				&
				Y\times Y\times Y
					&
		\end{tikzcd}
	\]
\end{proof}

\begin{lemma}
	Any left-sided $\Mono$-presentation
	\[
		\begin{tikzcd}[column sep=small]
				&
				A
				\ar[ld, "f"', tail]
				\ar[rd, "!"]
					&
			\\
			X
			\doublecell[rr, shift left=2.5ex]{\opcart}
			\sar[rr, "p"']
				&
					&
					1
		\end{tikzcd}
	\]
	exhibits $A$ as a tabulator of  $p$.
\end{lemma}
\begin{proof}
	\comment{ongoing}
\end{proof}

\begin{proposition}
	For a locally posetal discrete Cauchy cartesian equipment $\dbl{D}$, the following are equivalent.
	\begin{enumerate}
		\item
			$\dbl{D}$ has (left-sided) $\zero{M}$-comprehension scheme.
			for some stable system $\zero{M}$ on $\one{V}\dbl{D}$.
		\item
			$\dbl{D}$ has (left-sided) $\Mono$-comprehension scheme.
		\item
			$\dbl{D}$ has (left-sided) $\Mono$-presentations.
	\end{enumerate}
\end{proposition}
\begin{proof}
	\comment{ongoing}
\end{proof}

\begin{theorem}
	Let $\bi{B}$ be a locally posetal 2-category.
	The following are equivalent.
	\begin{enumerate}
		\item
			$\bi{B}$ is functionally complete and discrete.
		\item
			There exists a regular category $\one{E}$ such that $\bi{R}{el}(\one{E})$ is 2-equivalent to $\bi{B}$.
	\end{enumerate}
\end{theorem}

